How to Verify a Quantum Computation

We give a new theoretical solution to a leading-edge experimental challenge, namely to the verification of quantum computations in the regime of high computational complexity. Our results are given in the language of quantum interactive proof systems. Specifically, we show that any language in $\mathsf{BQP}$ has a quantum interactive proof system with a polynomial-time classical verifier (who can also prepare random single-qubit pure states), and a quantum polynomial-time prover. Here, soundness is unconditional--i.e., it holds even for computationally unbounded provers. Compared to prior work achieving similar results, our technique does not require the encoding of the input or of the computation; instead, we rely on encryption of the input (together with a method to perform computations on encrypted inputs), and show that the random choice between three types of input (defining a computational run, versus two types of test runs) suffices. Because the overhead is very low for each run (it is linear in the size of the circuit), this shows that verification could be achieved at minimal cost compared to performing the computation. As a proof technique, we use a reduction to an entanglement-based protocol; to the best of our knowledge, this is the first time this technique has been used in the context of verification of quantum computations, and it enables a relatively straightforward analysis.

==> tocspecial.tex <==
%% tocspecial.tex 2018-04-17   ToC style file
%------------------------------------------------------------------
% Filename: tocspecial.cls
% 
% This documentclass is intended for typesetting articles for the
% 
% Theory of Computing.
% 
% See http://theoryofcomputing.org for further details.
%
% Version 0.1 Initial combination of banners from previous style files.
% ------------------------------------------------------------------
%
%% Special issue banners:

\newcommand{\motwani}{Special issue in honor of Rajeev Motwani}
\newcommand{\boolean}{Special issue: Analysis of Boolean Functions}
\newcommand{\approxrandomBC}{Special issue: APPROX-RANDOM 2012}
\newcommand{\approxrandomBD}{Special issue: APPROX-RANDOM 2013}
\newcommand{\approxrandomBE}{Special issue: APPROX-RANDOM 2014}
\newcommand{\approxrandomBF}{Special issue: APPROX-RANDOM 2015}
\newcommand{\cccBF}{Special issue: CCC 2015}
\newcommand{\cccBG}{Special issue: CCC 2016}
\newcommand{\cccBH}{Special issue: CCC 2017}
\newcommand{\itcsBD}{Special issue: ITCS 2013}
%% explanation: BC = 2012 BD = 2013 ... CA = 2020 CB = 2021 ...

